Towards Richer Challenge Problems for Scientific Computing Correctness

Correctness in scientific computing (SC) is gaining increasing attention in the formal methods (FM) and programming languages (PL) community. Existing PL/FM verification techniques struggle with the complexities of realistic SC applications. Part of the problem is a lack of a common understanding between the SC and PL/FM communities of machine-verifiable correctness challenges and dimensions of correctness in SC applications. To address this gap, we call for specialized challenge problems to inform the development and evaluation of FM/PL verification techniques for correctness in SC. These specialized challenges are intended to augment existing problems studied by FM/PL researchers for general programs to ensure the needs of SC applications can be met. We propose several dimensions of correctness relevant to scientific computing, and discuss some guidelines and criteria for designing challenge problems to evaluate correctness in scientific computing.

==> eptcsdata.tex <==
\providecommand{\firstpage}{19}
\providecommand{\publicationstatus}{S.F.\ Siegel and G.\ Gopalakrishnan (Eds.):\\
International Workshop on Verification of\\
Scientific Software (VSS 2025)\\
EPTCS 432, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.432.4}{10.4204/EPTCS.432.4}}
\pdfoutput=1

